Generation through the lens of learning theory

We study generation through the lens of statistical learning theory. First, we abstract and formalize the results of Gold [1967], Angluin [1979], Angluin [1980] and Kleinberg and Mullainathan [2024] in terms of a binary hypothesis class defined over an abstract example space. Then, we extend the notion of "generation" from Kleinberg and Mullainathan [2024] to two new settings, we call "uniform" and "non-uniform" generation, and provide a characterization of which hypothesis classes are uniformly and non-uniformly generatable. As is standard in learning theory, our characterizations are in terms of the finiteness of a new combinatorial dimension termed the Closure dimension. By doing so, we are able to compare generatability with predictability (captured via PAC and online learnability) and show that these two properties of hypothesis classes are incompatible -- there are classes that are generatable but not predictable and vice versa. Finally, we extend our results to capture prompted generation and give a complete characterization of which classes are prompt generatable, generalizing some of the work by Kleinberg and Mullainathan [2024].

==> IILvUG.tex <==
\section{Uniform Generation vs. Identification in the Limit}

Equipped with a characterization of uniform generatability, we continue the comparison of generation and identification. It is not too hard to see that identifiability in the limit is harder then generatability in the limit -- any class identifiable in the limit is also generatable in the limit, but not vice versa. In the uniform case, one can show that uniform identifiability implies uniform generatability, but not vice versa. 

What about uniform generatability and identifiability in the limit? The following lemma shows that there exists a countable class that is uniformly generatable, but not identifiable in the limit. 

\begin{lemma}[Uniform Generatability $\centernot\implies$ Identifiability in the Limit] \label{lem:unifgennotiden} Let $\Xcal$ be countable. There exists a countable class $\Hcal \subseteq \{0, 1\}^{\Xcal}$ that satisfies the \emph{UUS} property,  is uniformly generatable, but not identifiable in the limit.
\end{lemma}

\begin{proof} Let $\Xcal = \mathbbm{Z}$ and $\Hcal = \{x \mapsto \mathbbm{1}\{x \in A \text{ or } x \leq 0\}: A \subset \mathbbm{N}, |A| < \infty \} \cup \{x \mapsto 1\}$. It is not hard to see that $\Hcal$ satisfies the UUS property and is countable. Moreover, $\Hcal$ is uniformly generatable since every hypothesis in $\Hcal$ contains $\mathbbm{Z}_{\leq 0}$ in its support.  Finally, to see that $\Hcal$ is not identifiable in the limit, consider the all-ones hypothesis $h(x) = 1$ and note that $h \in \Hcal$. It suffices to show that for every finite $A \subset \operatorname{supp}(h) = \mathbbm{Z}$, there exists $h^{\prime} \in \Hcal$ such that $A \subset \operatorname{supp}(h^{\prime})$ and $\operatorname{supp}(h^{\prime}) \subset \operatorname{supp}(h).$ To that end, fix some finite $A \subset \Zcal$ and consider the hypothesis $h^{\prime}(x) = \mathbbm{1}\{x \in A \text{ or } x \leq 0\}.$ Its not hard to see that $h^{\prime} \in \Hcal$, $A \subset \operatorname{supp}(h^{\prime})$, and $\operatorname{supp}(h^{\prime}) \subset \operatorname{supp}(h).$ Thus, $\Hcal$ is not identifiable in the limit, which completes the proof. 
\end{proof}

On the other hand, there also exists classes that are identifiable in the limit but not uniformly generatable!

\begin{lemma}[Identifiability in the Limit $\centernot\implies$ Uniform Generatability] \label{lem:identnotgen} Let $\Xcal$ be countable. There exists a countable class $\Hcal \subseteq \{0, 1\}^{\Xcal}$ that satisfies the \emph{UUS} property,  is identifiable in the limit, but not uniformly generatable.
\end{lemma}

\begin{proof} Let $\Hcal$ be the same hypothesis class from the proof of Lemma \ref{lem:nonunifvsunifgen}. In Lemma \ref{lem:nonunifvsunifgen}, we proved that $\operatorname{C}(\Hcal) = \infty$, which, using Theorem \ref{thm:unifgen}, gives that $\Hcal$ is not uniformly generatable. Thus, it only suffices to show that the conditions of Theorem \ref{thm:idenhard} hold for $\Hcal$. However, this is trivially true because for every $h_1, h_2 \in \Hcal$, we have that $\operatorname{supp}(h_1) \not\subset \operatorname{supp}(h_2)$ and $\operatorname{supp}(h_2) \not\subset \operatorname{supp}(h_1)$, thus condition (ii) in Theorem \ref{thm:idenhard} is always satisfied.  
% Pick any $h \in \Hcal$, and without any loss of generality, suppose $h \in \Hcal^{e}.$ We need to show that there exists a finite subset $S \subset \operatorname{supp}(h)$ such that for every $h^{\prime} \in \Hcal \setminus \{h\}$ for which $S \subset \operatorname{supp}(h^{\prime})$, then $\operatorname{supp}(h^{\prime}) \not\subset \operatorname{supp}(h).$ Let $d \in \mathbbm{N}$ be such that $\{\frac{d(d-1)}{2} + 1, , ..., \frac{d(d-1)}{2} + d\} \subset \operatorname{supp}(h)$ and take $S = \{\frac{d(d-1)}{2} + 1, ..., \frac{d(d-1)}{2} + d\}.$ Note that $|S| < \infty$. Moreover, there exists only one hypothesis $h^{\prime} \in \Hcal \setminus \{h\}$ such that $S \subset \operatorname{supp}(h^{\prime}).$ This is precisely the hypothesis $h^{\prime} \in \Hcal^o$ which also contains $S$, namely the hypothesis 
% $$h^{\prime} = h^o_d = \mathbbm{1}\Bigg\{x \in \Bigl\{\frac{d(d-1)}{2} + 1,  ..., \frac{d(d-1)}{2} + d\Bigl\} \text{ or } x \in O\Biggl\}.$$
% \noindent However, its not hard to see that $\operatorname{supp}(h^o_d) \not\subset \operatorname{supp}(h).$ This completes the proof, as our choice of $h \in \Hcal^e$ was arbitrary and a symmetric argument works for any $h \in \Hcal^o.$
\end{proof}

Together, Lemmas \ref{lem:unifgennotiden} and \ref{lem:identnotgen} show that uniform generatability and  identifiability in the limit are incompatible--there are cases where one is possible and the other is not. In the next section, we show that the same is also true when one compares prediction and generation. 
